Graph Transformer for Recommendation

This paper presents a novel approach to representation learning in recommender systems by integrating generative self-supervised learning with graph transformer architecture. We highlight the importance of high-quality data augmentation with relevant self-supervised pretext tasks for improving performance. Towards this end, we propose a new approach that automates the self-supervision augmentation process through a rationale-aware generative SSL that distills informative user-item interaction patterns. The proposed recommender with Graph TransFormer (GFormer) that offers parameterized collaborative rationale discovery for selective augmentation while preserving global-aware user-item relationships. In GFormer, we allow the rationale-aware SSL to inspire graph collaborative filtering with task-adaptive invariant rationalization in graph transformer. The experimental results reveal that our GFormer has the capability to consistently improve the performance over baselines on different datasets. Several in-depth experiments further investigate the invariant rationale-aware augmentation from various aspects. The source code for this work is publicly available at: https://github.com/HKUDS/GFormer.

==> model.tex <==
\section{Invariant Rationale-aware}
\label{sec:model}

\noindent\textbf{Graph-based Collaborative Filtering}. Inspired by the success of graph representation learning, many efforts~\cite{he2020lightgcn,wang2019neural,chen2020revisiting} aim at building graph-enhanced CF models for capturing high-order collaborative relations. Assume that there are $I$ users $\mathcal{U}=\{u_1, u_2,..., u_I\}$ and $J$ items $\mathcal{P}=\{p_1, p_2, ..., p_J\}$ in our recommendation scenario, and the observed user behaviors are represented by an interaction matrix $\textbf{A}\in\mathbb{R}^{I\times J}$. An element $a_{i,j}=1$ if an interaction between user $u_i$ and item $p_j$ is observed, and $a_{i,j}=0$ otherwise. In graph-based CF scenarios, the interaction matrix is transformed into an interaction graph $\mathcal{G}=\{\mathcal{V}, \mathcal{E}\}$, where $\mathcal{V}=\mathcal{U}\cup\mathcal{P}$ forms the node set, and $\mathcal{E}=\{e_{i,j}|a_{i,j}=1\}$ denotes the edge set corresponding to user-item interactions. With the above definitions, the graph-based CF can be abstracted as the prediction function: $\hat{y}_{i,j} = f(\mathcal{G}; \mathbf{\Theta})$, where $\hat{y}_{i,j}$ denotes the predicted score for the unknown interaction between user $u_i$ and item $p_j$. $\mathbf{\Theta}$ denotes the model parameters.
